What Aspects of Mobile Ads Do Users Care About? An Empirical Study of Mobile In-app Ad Reviews

In the mobile app ecosystem, developers receive ad revenue by placing ads in their apps and releasing them for free. While there is evidence that users do not like ads, we do not know what are the aspects of ads that users dislike nor if they dislike certain aspects of ads more than others. Therefore, in this paper, we analyzed the different topics of ad related complaints from users. In order to do this, we investigated app reviews that users gave for apps in the app store that were about ads. We manually examined a random sample set of 400 ad reviews to identify ad complaint topics. We found that most ad complaints were about user interface (UI) related topics and three topics were brought up the most often: the frequency with which ads were displayed, the timing of when ads were displayed, and the location of the displayed ads. Our results provide actionable information to software developers regarding the aspects of ads that are most likely to be complained about by users in their reviews.

==> Acknowledgement.tex <==
\section*{Acknowledgments}

This work was supported by National Science Foundation under Grant No. CCF-1619455. 


==> Analysis.tex <==
%\subsection{Confounding Variable Analysis}
\subsection{Best practices when all RQs are considered together}
\label{sec:conanalysis}




An app in our study could satisfy several ad usage aspects from our
RQs. For example, an app (Temperature app\footnote{Google Play app
  store: id=air.Android\_Temperature}) can have a banner ad (RQ1) that
is loaded in the landing page (RQ5). Hence, there is the chance that a
subset of the metrics that we examined in the RQs could be collinearly
related to another metric. In our previous analysis of pairwise
comparison (RQ1 - 6), we do not consider the effects of such
interaction between the metrics. Below we analyse the data using
proven statistical techniques to understand the interaction.

\subsubsection{Analysis Approach}

We collect the data required for this analysis from the data collected
for the RQs. In the dataset of this analysis, each row is an app that
we have analyzed in the RQs. Each column is the presence or absence of
a particular ad usage aspect in the corresponding app. For example the
first column is whether an app has a banner (0) or interstitial (1)
ad. Similar to this we calculate the complete set of ad usage aspects
(Interstitial or banner ads, Number of ads above or below median, One
or many ads per page, Area of ads above or below median, Height of ads
above or below median, Width of ads above or below median, Ad in the
landing page or not, Number of same ads above or below median,
Presence of ads in the top of the screen, Presence of ads in the
middle of the screen, Presence of ads in the bottom of the screen). We
consider these ad usage aspects as independent variables in our
analysis. The last independent variable that we considered was the
``Category of the app." We include the category to make sure that we
control for any bias based on the category of the app. Once we have
this dataset, we then build regression models to determine their
relationship among themselves and relationship to the average user
rating (dependent variable). We describe both these analysis below.

\subsubsection{Relationship between ad usage aspects}

In order to see if a certain combination of ad usage aspects are
linearly related to a particular aspect (e.g., all apps with banner
ads that are in the landing page always have them display in the
bottom), we rely on the redun method in the Hmisc package \cite{hmisc}
of the statistics tool R. In this analysis each ad usage aspect is
taken and a regression model is built with all the other ad usage
aspects. If the $R^2$ of the model is more than a threshold (default
value of 0.9 was used), then we consider that the particular ad usage
aspect under observation is a linear combination of the other ad usage
aspects.

On applying the redun analysis on the dataset, we found that the ad
usage aspect: `Area of ads above or below median' is a linear
combination of all the other variables with an $R^2$ value of 0.969
(almost perfect fit). \mei{This is not surprising since area is
  calculated as the product of height and width of the ad, and hence
  is likely related linearly.} Hence, we can drop this ad usage aspect
in our next analysis.

\subsubsection{Relationship between ad usage aspects and average user rating}

In this analysis we want to examine which ad usage aspects have the
most impact on average user rating when all other ad usage aspects are
also considered at the same time. \mei{Such an analysis gives the
  option to the developer to choose the most important ad usage aspect
  if they cannot apply all the best practices identified above.}
Since, we want to find the relative importance of ad usage aspects, we
build a random forest regression model. For this we used the
randomForest method from the R package, randomForest. By using the
importance method, we were able to determine the relative importance
of each ad usage aspect. The way such an analysis works is that, we
first build a random forest with all the ad usage aspects as
independent variables. Then we permute the values of one ad usage
aspect. We should see a fall in the model performance. The greater the
fall, the more important is the particular ad usage aspect. More on
this can be found here \cite{statisticalLearning}.

We applied this approach on our current dataset, and found that when
we controlled for all the ad usage aspects and the category of the
app, the top three most important ad usage aspects are: Ad in the
landing page or not, Number of same ads above or below median, and One
or many ads per page. From our RQs we know that ads in the landing
page, apps that repeat ads, and apps with more ads per page are
related to apps with lower ratings. Hence, we suggest that developers
be more careful about these three aspects in particular.


==> Background.tex <==
\section{Background}
\label{sec:background}

A \ac{man}, is a company that connects advertisers to apps that
display advertisements. \acp{man} provide sophisticated frameworks and
infrastructure (\eg ad libraries) to deliver ads and allow developers
to incorporate ads into their app. This process starts with developers
registering an \emph{ad profile} that provides them with a unique ID
that corresponds to their app.  Using this ID, developers can
configure the types of ads they want their app to receive and
characteristics about those ads.  The exact configurations available
vary by ad networks, but generally developers are able to choose
between different size ads and different types of content.  Ads that
occupy the full screen are also called \emph{interstitial ads} and
require the user to view the ad for a time interval or click a close
button to return to the app.  Users often call these ``popup'' ads,
since they appear in the middle of an execution.  Ads that occupy less
than a full screen are generally referred to as \emph{banner ads}.
These typically show up as horizontal boxes that span the screen's
width, but only occupy a portion of the vertical space available on
the screen.  They allow a user to interact with the other visible
parts of the app's \ac{ui} while the ad is being displayed.

Developers typically have a lot of control over how, where, and when
to display ads in their app.  Ads delivered from the \ac{man} may be
in the form of an image, text, or video.  Developers can use different
\ac{ui} containers to position and show the ads on the screen.
Developers may choose certain preset sizes for ads.  For example
Google AdMob allows developers to request ads with different preset
sizes, such as \textit{FULL BANNER}, \textit{LARGE BANNER}, and
\textit{SMART BANNER}. Ads that are pure images are somewhat unusual,
but can be displayed in any way that Android allows \acp{ui} to
display images.  More common are ads in the form of
HTML/CSS/JavaScript code, which are displayed in an Android \ac{ui}
component called a \texttt{WebView}. A developer can position
\texttt{WebView} components to display the ads they receive from the
ad network. A \ac{ui} layout in Android defines the visual structure
for a user interface. A \ac{ui} layout can be created by instantiating
the \ac{ui} components at runtime or by configuring an XML based
layout file that will be loaded and rendered at runtime. The XML file
is traditionally the most straightforward and preferred method for
extracting or representing an app's \ac{ui} layout. Many popular
Android \ac{ui} automator tools, such as \textit{Hierarchy Viewer} or
\ac{uiat}, can extract a detailed XML layout file from an app that
represents the \ac{ui}, regardless of how the \ac{ui} was generated.



==> Category.tex <==
\subsection{RQ 7: \rqg}
\label{sec:category}

\rqsec{Approach}: In our automated experiments, we did not run PUMA on game apps. This is because they required many non-deterministic UI actions. To the best of our knowledge, out of the up-to-date tools for testing, there is no ideal tool to interact with game apps. We manually interacted with \jp{game-app-number} game apps for four minutes, and followed the same steps as in other RQs to obtain the statisitics. Then we compared the game apps with non-game apps for each of the above RQs.



==> DiscussionTable.tex <==

\begin{table}[t]\scriptsize
  \caption{Summary of the key findings of the paper expressed as
    suggestions for developers.}
\label{tab:dis}
\centering
\begin{tabular}{p{1cm}p{6.6cm}}
  \toprule
  \textbf{RQ} & \textbf{Take-away points for developers} \\
  \midrule

  RQ1 & Apps without interstitial ads (\ie only banner ads) typically
  have a higher rating than those apps that have at least one
  interstitial ad. \\

  \midrule

  RQ2 & Developers need to carefully control the number of ads among
  all activities and the number of ads within one page. Apps with ads
  in more than half the pages and more than one ad per page typically
  have a lower rating. \\

  \midrule

  RQ3 & Ads with a height of more than 150p typically have a lower
  rating. However, our study shows no similar statistical evidence for
  the width of ads. \\

  \midrule

  RQ4 & Higher rated apps typically have ads in the top of the screen
  rather than the bottom or middle of the screen. \\

  \midrule

  RQ5 & Lower rated apps typically include ads in the landing page.\\ %Inclusion of ads in the landing pages risks receiving negative ad reviews and lower user ratings. \\

  \midrule

  RQ6 & Apps with a lower rating usually repeat almost half of their ads. \\ %To much content repetition (with the median 0.5 in our study) of ads can lead to lower ratings from users. \\

\bottomrule
\end{tabular}
\end{table}


==> Makefile <==
MAIN = paper
TARGET = $(MAIN).pdf
FIGURE_DIR=figs

SOURCES = $(wildcard *.tex *.bib $(FIGURE_DIR)/*)
GS_OPTIONS="-sDEVICE=pdfwrite -dEmbedAllFonts=true -dPDFSETTINGS=/prepress"

check: $(TARGET)
		svn status|grep ^?|awk '{print "\n\t" $$2 " -- Not under version control\n"}'
		svn status|grep ^[MA]|awk 'BEGIN {print ""} {print "\t" $$2 " -- updated but not committed"} END {print ""}'

$(TARGET): $(SOURCES)
		GS_OPTIONS=$(GS_OPTIONS) rubber --pdf -Wrefs $(MAIN)

clean:
		rubber --pdf --clean $(MAIN)

.SILENT: 


==> cutText.tex <==
\eat{
RQ3: are the problems related to ad complaints really existed in the corresponding app? (Qualitative study)
Information related to experiments (e.g., smartphones, and apps).
Include the content of the reviews instead of only the ratings.

The reason we used the old version of the operating system is that it was more compatible with the corresponding apk files that the latest version of the system.

Ads are not displayed in the original version due to old ad libraries, but shown in the latest version. This indirectly shows developers did not address ad complaints among app reviews.

For apps that need registration before accessing to the landing page, we registered with a new account to access app's complete functionality. Note that few apps failed the registration due to network connection.

ad block function: in some cases (ad server/ad delivery mechanism/poor network conditions), ads cannot be displayed, which blocks the loading of the app's main functions. ads in paid version were not handled. Slow problem depends on the OS, hardware and context (\eg running multiple apps at the same time). It is challenging to get the recurrent scenario in the ad review.

Some apps had ad area on most pages but no ads were displayed. Some apps crashed after the launch or during the play (due to the incompatibility or other issues).

The ad content is different during different time, and it can affect the user experience if the content is similar to app content.

Multiple banners on the same page, but one time one ad was displayed. Only through scrolling can we see all the ads. They could have different sizes.

No ad in old version, ads in the latest version: maybe old version could not receive ad data from ad servers.

For apps that have a list of information (\eg news), ads are displayed among app content. When scrolling down, we can see different ads. On one page, only ad is displayed. The list is dynamically loaded.

Due to out-dated version of ad libraries (or ad unit id updated), ads may not be retrieved and displayed properly, which makes the app crash (\textit{``Horrible, ad comes up when I hit resume game takes me to same place"}). It is also possible that after reviewing ad complaints, developers deactivate ads in their apps. If these ads are the same among all versions, then the ads in the original version will not be displayed either. In this case, we cannot verify ad complaints. The latest version is not available anymore on Google Play app store and we cannot verify ad complaints in the latest version either. Non \ac{ui} related, and non ad complaints, and other

For the news app, the ad content is dynamically loaded during the runtime. The ads are controlled by the server and their sizes are various. In other words, there is not an separate view object for ads, unlike traditional apps. Some apps not only have banner ad but also dynamic ad among content (\ie multiple ads on the same page)

Not find the problem (\eg ad sexy content) in the app (old or latest), but find new problems (\eg too many ads, intrusive, multiple ads on the same page) not mentioned in the review.

Reasons for missing ad problems in apps: need upgrade before entering the landing page, out dated ad libraries, different ad content determined by ad networks during different time periods, app crash, app landing page with not content

For popular apps (\eg angrybirds), developers addressed all ad problems in the latest version.

Threat: triggering the problem in the ad review may require some specific steps (\eg ad only shown after a long playing game) and we may miss such workload during the qualitative analysis. We may have a different thought on the words used by users. For example, few users used ``popup every 5 seconds" for banners to show the frequently refresh banner ads.
}

\begin{table}[]
\centering
\caption{Clustered topics of three NLP based techinques}
\label{tab:perf}
\begin{tabular}{|c|c|c|}
\hline
         & \begin{tabular}[c]{@{}c@{}}UI topics\\ (\# \textit{auto}/\# \textit{manual})\end{tabular} & \begin{tabular}[c]{@{}c@{}}Non-UI topics\\ (\# \textit{auto}/\# \textit{manual})\end{tabular} \\ \hline
K-means  & 7/9 & 2/7 \\ \hline
LDA      & 7/9 & 5/7 \\ \hline
Word2Vec & 9/9 & 6/7 \\ \hline

\end{tabular}
\end{table}


\eat{
\begin{table*}[h]
\centering
\caption{Large-scale ad complaint topics for each app category}
\label{tab:large-scale-topics}
\begin{tabular}{|l|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{App category}} & \multicolumn{1}{c|}{\textbf{Top five UI topics}}   & \multicolumn{1}{c|}{\textbf{Top five Non-UI topics}} \\ \hline
ARCADE                                      & time, frequency, location, intrusive, blank        & auto, block, crash, slow, paid                       \\ \hline
BOOKS\_AND\_REFERENCE                       & time, intrusive, frequency, content, location      & paid, auto, block, crash, slow                       \\ \hline
BRAIN                                       & frequency, intrusive, location, time, content      & auto, block, crash, slow, paid                       \\ \hline
BUSINESS                                    & time, location, frequency, intrusive, popup        & paid, auto, block, slow, crash                       \\ \hline
CARDS                                       & time, frequency, intrusive, location, blank        & auto, block, crash, paid, slow                       \\ \hline
CASUAL                                      & frequency, time, location, intrusive, content      & block, auto, crash, paid, slow                       \\ \hline
COMICS                                      & time, location, popup, frequency, notification     & crash, paid, auto, block, slow                       \\ \hline
COMMUNICATION                               & time, frequency, location, intrusive, blank        & auto, block, slow, paid, crash                       \\ \hline
EDUCATION                                   & time, location, frequency, popup, content          & paid, block, auto, crash, battery                    \\ \hline
ENTERTAINMENT                               & time, frequency, location, intrusive, content      & slow, crash, block, auto, paid                       \\ \hline
FINANCE                                     & time, location, frequency, intrusive, content      & paid, block, auto, crash, slow                       \\ \hline
HEALTH\_AND\_FITNESS                        & frequency, location, time, intrusive, size         & auto, block, paid, crash, slow                       \\ \hline
LIBRARIES\_AND\_DEMO                        & frequency, time                                    & paid, auto                                           \\ \hline
LIFESTYLE                                   & time, frequency, location, intrusive, content      & paid, block, crash, auto, slow                       \\ \hline
MEDIA\_AND\_VIDEO                           & time, frequency, location, blank, content          & auto, block, slow, crash, paid                       \\ \hline
MEDICAL                                     & time, location, frequency, popup, notification     & paid, block, crash, auto, slow                       \\ \hline
MUSIC\_AND\_AUDIO                           & time, frequency, notification, blank, intrusive    & block, crash, auto, paid, slow                       \\ \hline
NEWS\_AND\_MAGAZINES                        & time, frequency, location, intrusive, content      & auto, block, crash, paid, slow                       \\ \hline
PERSONALIZATION                             & time, frequency, location, intrusive, popup        & auto, paid, block, slow, crash                       \\ \hline
PHOTOGRAPHY                                 & time, frequency, location, intrusive, popup        & auto, block, crash, paid, slow                       \\ \hline
PRODUCTIVITY                                & time, frequency, intrusive, location, content      & auto, slow, block, crash, paid                       \\ \hline
RACING                                      & time, location, frequency, popup, intrusive        & block, crash, paid, auto, slow                       \\ \hline
SHOPPING                                    & time, location, frequency, size, notification      & paid, auto, block, slow, crash                       \\ \hline
SOCIAL                                      & time, frequency, location, intrusive, content      & auto, block, slow, crash, paid                       \\ \hline
SPORTS                                      & time, frequency, location, blank, intrusive        & auto, block, slow, crash, paid                       \\ \hline
SPORTS\_GAMES                               & time, location, frequency, intrusive, popup        & block, paid, crash, auto, slow                       \\ \hline
TOOLS                                       & time, frequency, location, intrusive, content      & auto, block, slow, crash, paid                       \\ \hline
TRANSPORTATION                              & time, location, frequency, notification, intrusive & paid, auto, block, crash, slow                       \\ \hline
TRAVEL\_AND\_LOCAL                          & time, location, frequency, intrusive, size         & paid, auto, slow, block, crash                       \\ \hline
WEATHER                                     & time, intrusive, frequency, location, size         & paid, block, slow, auto, crash                       \\ \hline
\end{tabular}
\end{table*}
}


